Covariate Balancing Propensity Score by Tailored Loss Functions

In observational studies, propensity scores are commonly estimated by maxi- mum likelihood but may fail to balance high-dimensional pre-treatment covariates even after specification search. We introduce a general framework that unifies and generalizes several recent proposals to improve covariate balance when designing an observational study. In- stead of the likelihood function, we propose to optimize special loss functions---covariate balancing scoring rules (CBSR)---to estimate the propensity score. A CBSR is uniquely determined by the link function in the GLM and the estimand (a weighted average treatment effect). We show CBSR does not lose asymptotic efficiency to the Bernoulli likelihood in estimating the weighted average treatment effect compared, but CBSR is much more robust in finite sample. Borrowing tools developed in statistical learning, we propose practical strategies to balance covariate functions in rich function classes. This is useful to estimate the maximum bias of the inverse probability weighting (IPW) estimators and construct honest confidence interval in finite sample. Lastly, we provide several numerical examples to demonstrate the trade-off of bias and variance in the IPW-type estimators and the trade-off in balancing different function classes of the covariates.

==> realdata.tex <==
The next example is the National Supported Work (NSW) Demonstration which was previously analyzed by
\citet{lalonde1986evaluating,dehejia1999causal,smith2005does} and
many other authors. The NSW Demonstration provided
transitional and subsidized work experience for a period of
6--18 months to individuals who had faced economic and social problems
prior to the enrollment in the program. The pre-treatment covariates
include earnings, education, age, ethnicity, and
marital status, and the outcome of interest in
\citet{lalonde1986evaluating} is the post-intervention earnings in 1978.
We use the experimental subsample taken by
\citet{dehejia1999causal} to demonstrate our methods, which include
$185$ treated and $260$ control observations that joined the program
early enough for the retrospective earnings information in the year
1974. To evaluate the non-experimental methods, we use the
Current Population Survey (CPS) data extracted by
\citet{lalonde1986evaluating} as the control group, which contain
$15992$ observations. The
reader is referred to the previous articles listed in this paragraph for more
detailed information on this dataset.

The observational methods are evaluated in two scenarios:
\begin{enumerate}[label=\arabic*.]
\item Compare the experimental treated group with the non-experimental
  control group. The average treatment effect estimators can be
  compared with the experimental benchmark, which is 1794.3 (standard
  error 632.9) by a linear regression of the earnings in 1978 on the
  treatment assignment.
\item Compare the experimental control group with the non-experimental
  control group. Since both groups did not receive treatment, the
  treatment effect is always zero (the null case in \Cref{sec:impl-covar-balance}).
\end{enumerate}
Since the non-experimental control group is very large and has very
different covariate distribution to the experimental group, we only
consider the average treatment effect on the treated (ATT)
in this example. Using \Cref{tab:scoring-rule}, the CBSR rule in this
case is $S_{0,-1}$.

First, we apply the forward stepwise regression in
\Cref{alg:fstep}. To generate predictors $\phi(X)$, we use all the
discrete covariates (race, married, no degree, no earning in 1974, no
earning in 1975), all the continuous covariates (age, year of
education, earning in 1974, earning in 1975) and their squares, and
the first-order interactions of all these variables. This results in
a $94$-dimensional vector $\phi$ of predictors. In each scenario, two
scoring rules, the Bernoulli likelihood $S_{0,0}$ and the covariate
balancing scoring rule $S_{0,-1}$, are used, and the covariate
imbalance and the estimator $\hat{\tau}$ are plotted along the
stepwise path.

The results of the forward stepwise regressions can be found in
\Cref{fig:lalonde-fstep-1}. Compared to the Bernoulli likelihood, CBSR requires a stronger condition for the existence of the
solution \citep{zhao2015}, so in both scenarios CBSR stops early ($71$ steps in scenario 1 and $23$ steps in
scenario 2). Nevertheless, CBSR is much better at reducing covariate imbalance as shown in
\Cref{fig:lalonde-fstep-1-imba,fig:lalonde-fstep-2-imba}. In fact,
at least $10$ predictors have standardized difference greater than
$20\%$ across the entire path when the Bernoulli likelihood is used,
while some authors have suggested that a standardized difference above
10\% can be deemed substantial
\citep{normand2001validating,austin2015moving}. When a two-sample
t-test is used to compare the mean of the predictors, less than $20\%$
of the $94$ tests are insignificant with the Bernoulli likelihood,
also implying insufficient covariate balance. On the contrary, CBSR successfully balances most predictors
in both scenarios.

\Cref{fig:lalonde-fstep-1-est,fig:lalonde-fstep-2-est} show
the estimate of ATT along the path. Interesting, by just including the first predictor most of
the bias of estimating ATT is corrected. Both scoring rules give similar
estimates and are consistent with the experimental
benchmarks. However, as discussed above, the weights generated by
maximizing the Bernoulli likelihood are unacceptable to many applied
researchers. Switching to CBSR solves this
problem, though the ATT estimates are not very different in this
particular example. Additionally, when using CBSR the standard error of $\hat{\tau}$ is smaller. This can
be understood from the remark in the supplementary file that CBSR
tries to avoid large weights.

% Next, we apply the forward stagewise regression in
% \Cref{alg:fstage} with the same $94$ predictors (each predictor is
% normalized to have sample variance equal to $1$). The results are shown
% in \Cref{fig:lalonde-fstage-1}. In general, these
% plots are similar to those using the forward stepwise regression: only
% CBSR generates covariate balancing weights, though the ATT estimates are not too
% different. There are still two notable differences. First, the curves
% in \Cref{fig:lalonde-fstage-1-est,fig:lalonde-fstage-2-est} are smoother than those in
% \Cref{fig:lalonde-fstep-1-est,fig:lalonde-fstep-2-est}. This is
% because at one time the forward stagewise regression only increases one
% coefficient by a small amount. Second, when using the Bernoulli
% likelihood the covariate imbalance not monotonically decreasing. In
% fact, after $800$ steps the predictors start to become more imbalanced
% due to overfitting the propensity score. CBSR does not suffer from
% overfitting as the standardized differences keep decreasing as the model
% gets more complicated.

Next, we apply the kernel method in \Cref{sec:kernel-methods} and
the results are presented in
\Cref{fig:lalonde-kernel-1}. We use the Gaussian
kernel $K(x,x') = \exp(-\sigma \|x - x'\|^2)$ with $\sigma = 0.15$ and
$x = (\texttt{black}$, $\texttt{hispanic}$, $\texttt{no\,degree}$,
$\texttt{married}$, $\texttt{age} / 5$, $\texttt{education} / 3$,
$\texttt{re74} / 4000$, $\texttt{re75} / 4000)$.
The first four entries in $x$ are indicator variables, and
$\texttt{re74}$ ($\texttt{re75}$) stands for the annual earning of the
person in the year 1974 (1975). Because the kernel matrix is a large $n
\times n$ matrix, we use the subsample CPS2 extracted by
\citet{dehejia1999causal} that contains $n = 2369$ non-experimental controls. Overall, these two plots are
similar to those for the forward stepwise regressions.
Notice that the confidence intervals of ATT are wider when
using the kernel method. This loss of efficiency is compensated by the improved
robustness, as the propensity score weights approximately balance infinite many covariate
functions (\Cref{sec:kernel-methods}).

\begin{figure}[p]
  \centering
  \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width =
    \textwidth]{../figure/lalonde_fstep_exp_treat_imba}
    \caption{\small Covariate imbalance: experimental
    treatment vs.\ non-experimental control.}
    \label{fig:lalonde-fstep-1-imba}
  \end{subfigure}
  \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width =
    \textwidth]{../figure/lalonde_fstep_exp_control_imba}
    \caption{\small Covariate imbalance: experimental
    control vs.\ non-experimental control.}
    \label{fig:lalonde-fstep-2-imba}
  \end{subfigure} \\
  \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width =
    \textwidth]{../figure/lalonde_fstep_exp_treat_est}
    \caption{\small Estimate of ATT: experimental
    treatment vs.\ non-experimental control.}
    \label{fig:lalonde-fstep-1-est}
  \end{subfigure}
  \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width =
    \textwidth]{../figure/lalonde_fstep_exp_control_est}
    \caption{\small Estimate of ATT: experimental
    control vs.\ non-experimental control.}
    \label{fig:lalonde-fstep-2-est}
  \end{subfigure}
  \caption{Forward stepwise regressions for the
    \cite{lalonde1986evaluating} dataset. Top panels: Covariate
    imbalance is in terms of standardized difference. The curves in the plot are the $1$st, $5$th, $10$th,
      and $25$th largest standardized difference among the $94$
      predictors (solid lines), and the percentage of insignificant two-sample
      t-tests comparing the mean of each predictor in the treatment
      and the weighted control (dotted line). Bottom panels: estimated
    ATT with 95\% confidence interval.}
  \label{fig:lalonde-fstep-1}
\end{figure}

% \begin{figure}[ht]
%   \centering
%   \begin{subfigure}[b]{\textwidth}
%     \includegraphics[width =
%     \textwidth]{../figure/lalonde_fstep_exp_control_imba}
%     \caption{Covariate imbalance in terms of standardized
%       difference. The curves in the plot are the $1$st, $5$th, $10$th,
%       and $25$th largest standardized difference among the $94$
%       predictors (solid lines), and the percentage of insignificant two-sample
%       t-tests comparing the mean of each predictor in the treatment
%       and the weighted control (dotted line).}
%     \label{fig:lalonde-fstep-2-imba}
%   \end{subfigure} \\
%   \begin{subfigure}[b]{\textwidth}
%     \includegraphics[width =
%     \textwidth]{../figure/lalonde_fstep_exp_control_est}
%     \caption{Estimate of ATT with $95\%$ confidence interval.}
%     \label{fig:lalonde-fstep-2-est}
%   \end{subfigure}
%   \caption{Forward stepwise regressions in the second scenario: experimental
%     control vs.\ non-experimental control.}
%   \label{fig:lalonde-fstep-2}
% \end{figure}

% \begin{figure}[p]
%   \centering
%   \begin{subfigure}[b]{0.48\textwidth}
%     \includegraphics[width =
%     \textwidth]{../figure/lalonde_fstage_exp_treat_imba}
%     \caption{Covariate imbalance: experimental
%     treatment vs.\ non-experimental control.}
%     \label{fig:lalonde-fstage-1-imba}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.48\textwidth}
%     \includegraphics[width =
%     \textwidth]{../figure/lalonde_fstage_exp_control_imba}
%     \caption{Covariate imbalance: experimental
%     control vs.\ non-experimental control.}
%     \label{fig:lalonde-fstage-2-imba}
%   \end{subfigure} \\
%   \begin{subfigure}[b]{0.48\textwidth}
%     \includegraphics[width =
%     \textwidth]{../figure/lalonde_fstage_exp_treat_est}
%     \caption{Estimate of ATT: experimental
%     treatment vs.\ non-experimental control.}
%     \label{fig:lalonde-fstage-1-est}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.48\textwidth}
%     \includegraphics[width =
%     \textwidth]{../figure/lalonde_fstage_exp_control_est}
%     \caption{Estimate of ATT: experimental
%     control vs.\ non-experimental control.}
%     \label{fig:lalonde-fstage-2-est}
%   \end{subfigure}
%   \caption{Forward stagewise regressions for the
%     \cite{lalonde1986evaluating} dataset. Top panels: Covariate
%     imbalance is in terms of standardized difference. The curves in the plot are the $1$st, $5$th, $10$th,
%       and $25$th largest standardized difference among the $94$
%       predictors (solid lines), and the percentage of insignificant two-sample
%       t-tests comparing the mean of each predictor in the treatment
%       and the weighted control (dotted line). Bottom panels: estimated
%     ATT with 95\% confidence interval.}
%   \label{fig:lalonde-fstage-1}
% \end{figure}


% \begin{figure}[ht]
%   \centering
%   \begin{subfigure}[b]{\textwidth}
%     \includegraphics[width =
%     \textwidth]{../figure/lalonde_fstage_exp_treat_imba}
%     \caption{\small Covariate imbalance in terms of standardized
%       difference. The curves in the plot are the $1$st, $5$th, $10$th,
%       and $25$th largest standardized difference among the $94$
%       predictors (solid lines), and the percentage of insignificant two-sample
%       t-tests comparing the mean of each predictor in the treatment
%       and the weighted control (dotted line).}
%     \label{fig:lalonde-fstage-1-imba}
%   \end{subfigure} \\
%   \begin{subfigure}[b]{\textwidth}
%     \includegraphics[width =
%     \textwidth]{../figure/lalonde_fstage_exp_treat_est}
%     \caption{\small Estimate of ATT with $95\%$ confidence interval.}
%     \label{fig:lalonde-fstage-1-est}
%   \end{subfigure}
%   \caption{Forward stagewise regressions ($\epsilon = 0.005$) in the first scenario: experimental
%     treatment vs.\ non-experimental control.}
%   \label{fig:lalonde-fstage-1}
% \end{figure}

% \begin{figure}[ht]
%   \centering
%   \begin{subfigure}[b]{\textwidth}
%     \includegraphics[width =
%     \textwidth]{../figure/lalonde_fstage_exp_control_imba}
%     \caption{Covariate imbalance in terms of standardized
%       difference. The curves in the plot are the $1$st, $5$th, $10$th,
%       and $25$th largest standardized difference among the $94$
%       predictors (solid lines), and the percentage of insignificant two-sample
%       t-tests comparing the mean of each predictor in the treatment
%       and the weighted control (dotted line).}
%     \label{fig:lalonde-fstage-2-imba}
%   \end{subfigure} \\
%   \begin{subfigure}[b]{\textwidth}
%     \includegraphics[width =
%     \textwidth]{../figure/lalonde_fstage_exp_control_est}
%     \caption{Estimate of ATT with $95\%$ confidence interval.}
%     \label{fig:lalonde-fstage-2-est}
%   \end{subfigure}
%   \caption{Forward stagewise regressions ($\epsilon = 0.005$) in the second scenario: experimental
%     control vs.\ non-experimental control.}
%   \label{fig:lalonde-fstage-2}
% \end{figure}


\begin{figure}[p]
  \centering
  \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width =
    \textwidth]{../figure/lalonde_kernel_exp_treat_imba}
    \caption{\small Covariate imbalance: experimental
    treatment vs.\ non-experimental control.}
    \label{fig:lalonde-kernel-1-imba}
  \end{subfigure}
  \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width =
    \textwidth]{../figure/lalonde_kernel_exp_control_imba}
    \caption{\small Covariate imbalance: experimental
    control vs.\ non-experimental control.}
    \label{fig:lalonde-kernel-2-imba}
  \end{subfigure} \\
  \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width =
    \textwidth]{../figure/lalonde_kernel_exp_treat_est}
    \caption{\small Estimate of ATT: experimental
    treatment vs.\ non-experimental control.}
    \label{fig:lalonde-kernel-1-est}
  \end{subfigure}
  \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width =
    \textwidth]{../figure/lalonde_kernel_exp_control_est}
    \caption{\small Estimate of ATT: experimental
    control vs.\ non-experimental control.}
    \label{fig:lalonde-kernel-2-est}
  \end{subfigure}
  \caption{Reproducing kernel method for the
    \cite{lalonde1986evaluating} dataset. Top panels: Covariate
    imbalance is in terms of standardized difference. The curves in the plot are the $1$st, $5$th, $10$th,
      and $25$th largest standardized difference among the $94$
      predictors (solid lines), and the percentage of insignificant two-sample
      t-tests comparing the mean of each predictor in the treatment
      and the weighted control (dotted line). Bottom panels: estimated
    ATT with 95\% confidence interval.}
  \label{fig:lalonde-kernel-1}
\end{figure}


% \begin{figure}[!ht]
%   \centering
%   \begin{subfigure}[b]{\textwidth}
%     \includegraphics[width =
%     \textwidth]{../figure/lalonde_kernel_exp_treat_imba}
%     \caption{Covariate imbalance in terms of standardized
%       difference. The curves in the plot are the $1$st, $5$th, $10$th,
%       and $25$th largest standardized difference among the $94$
%       predictors (solid lines), and the percentage of insignificant two-sample
%       t-tests comparing the mean of each predictor in the treatment
%       and the weighted control (dotted line).}
%     \label{fig:lalonde-kernel-1-imba}
%   \end{subfigure} \\
%   \begin{subfigure}[b]{\textwidth}
%     \includegraphics[width =
%     \textwidth]{../figure/lalonde_kernel_exp_treat_est}
%     \caption{Estimate of ATT with $95\%$ confidence interval.}
%     \label{fig:lalonde-kernel-1-est}
%   \end{subfigure}
%   \caption{Kernel regressions in the first scenario: experimental
%     treatment vs.\ non-experimental control.}
%   \label{fig:lalonde-kernel-1}
% \end{figure}

% \begin{figure}[!ht]
%   \centering
%   \begin{subfigure}[b]{\textwidth}
%     \includegraphics[width =
%     \textwidth]{../figure/lalonde_kernel_exp_control_imba}
%     \caption{Covariate imbalance in terms of standardized
%       difference. The curves in the plot are the $1$st, $5$th, $10$th,
%       and $25$th largest standardized difference among the $94$
%       predictors (solid lines), and the percentage of insignificant two-sample
%       t-tests comparing the mean of each predictor in the treatment
%       and the weighted control (dotted line).}
%     \label{fig:lalonde-kernel-2-imba}
%   \end{subfigure} \\
%   \begin{subfigure}[b]{\textwidth}
%     \includegraphics[width =
%     \textwidth]{../figure/lalonde_kernel_exp_control_est}
%     \caption{Estimate of ATT with $95\%$ confidence interval.}
%     \label{fig:lalonde-kernel-2-est}
%   \end{subfigure}
%   \caption{Kernel regressions in the second scenario: experimental
%     control vs.\ non-experimental control.}
%   \label{fig:lalonde-kernel-2}
% \end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> simulation.tex <==
This example due to \citet{Kang2007} is also used to
generate \Cref{fig:fstep-imba} in the Introduction. The
artificial
dataset consists of i.i.d.\ random variables $({X}_i, {Z}_i, T_i,
Y_i),~ i=1,\ldots,n $, where ${X}_i$, $Y_i$ and
$T_i$ are always observed and ${Z}_i$ is never observed. To generate
this data set, ${X}_i$ is a $4$-dimensional vector distributed as
$\mathrm{N}(0,I_4)$; ${Z}_i$ is computed by first applying the following  transformation:
\begin{align*}
  Z_{i1} = \exp(X_{i1}/2), ~Z_{i2} = X_{i2}/(1 + \exp(X_{i1})) +
  10,\\
  Z_{i3}= (X_{i1}X_{i3} + 0.6)^3,~ Z_{i4} = (X_{i2} + X_{i4} +
  20)^2,
\end{align*}
and then normalizing individual variables of ${Z}$ to have sample mean $0$
and variance $1$.

There are in total four settings in this example. In the first setting
(top-left panel in \Cref{fig:comparison-KS}), $Y_i$ is generated by
$Y_i = g({X},T_i)$ without any additional noise, where
\[
g({X},0) =
210 + 27.4 X_{i1} + 13.7 X_{i2} + 13.7 X_{i3} + 13.7 X_{i4},
\]
and $g({X},1)$ is either equal to $g({X},0)$ (column ``zero'' in
\Cref{fig:comparison-KS}) or $g({X},0) + 10$ (column ``constant'' in
\Cref{fig:comparison-KS}). The
true propensity scores are generated by the logistic model $p(X_i) =
l^{-1}(f(X_i)),~f(X_i) = -X_{i1} + 0.5 X_{i2} - 0.25 X_{i3} -0.1
X_{i4}$. In this setting, both $Y$ and $T$ can be correctly modeled by
(generalized) linear model of the observed covariates ${X}$.
In the other settings, at least one of the propensity score model $f$ and
the outcome regression model $g$ is non-linear in ${X}$. In order to
achieve this, the data generating process described above is altered
such that $Y$ or $T$ (or both) is linear in the unobserved ${Z}$
instead of the observed ${X}$, though the parameters are kept the
same. For each setting, $200$ replicas of dataset of size $n = 200$ are
drawn. The logistic link function is always used and different scoring rules
in the Beta-family \eqref{eq:beta-family} are applied. The predictor vector
$\phi$ used is $\phi(X) =
(X_1,X_1^2,X_2,X_2^2,X_3,X_3^2,X_4,X_4^2)$.
After a propensity score model
is obtained, we use the
normalized IPW estimator $\hat{\tau}_{-1,-1}^{*}$ to estimate ATE and
$\hat{\tau}_{0,-1}^{*}$ to estimate ATT. The covariate imbalance with
respect to $\phi$ is shown earlier in \Cref{fig:fstep-imba}.

\begin{figure}[t]
  \centering
  \includegraphics[width = 0.9\textwidth]{../figure/comparison}
  \caption{Estimate of average treatment effects (ATE or ATT) using
    different scoring rules under the four settings. The four boxes in
    each group with different colors correspond to the Beta scoring rule
    \eqref{eq:beta-family} with 1.\ $\alpha = \beta = -1$; 2.\ $\alpha = 0,
    \beta = -1$; 3.\ $\alpha = \beta = 0$; 4.\ $\alpha = \beta = 0$
    (Bernoulli likelihood). In the first and third boxes, the
    inverse probability weights corresponding to ATE ($\alpha = \beta
    = -1$ in equation \eqref{eq:gipw-alpha-beta}) is used. In the second and
    fourth boxes, the inverse probability weights corresponding to ATT
    ($\alpha = 0, \beta = -1$) is used. The gray dashed lines
    correspond to the true treatment effect: $0$ for group ``zero''
    and $10$ for group ``constant''.}
  \label{fig:comparison-KS}

\end{figure}

\Cref{fig:comparison-KS} shows the boxplots of these estimates. It is clear that the covariate balancing scoring
rules (CBSR) generate much more stable
estimates than the Bernoulli likelihood (MLE). In the two left panels the true logit $f$ is
linear in ${X}$ so the propensity score model is correctly
specified. In the two top panels the true outcome regression function $g_0$ is linear in ${X}$. As
expected, the weighting estimators given by CBSR are unbiased across
these three panels besides the bottom-right one. If instead the
Bernoulli likelihood criterion is used to estimate the propensity
score model, the weighting estimator is biased when $f$ is non-linear
in ${X}$ (right panels). Even if $f$
is linear in ${X}$ so the propensity score model is correctly specified, the CBSR estimators have much smaller
variance than MLE. Lastly, in the bottom-right panel where both $f$ and
$g$ are non-linear, CBSR still has smaller bias and variance compared
to MLE.

Next we test the adaptive strategies described in
\Cref{sec:extensions}. Here we consider three adaptive
strategies---forward stepwise regression and two reproducing kernel
Hilbert space (RKHS) regressions. In the forward stepwise regression, we
use all the two-way interactions of degree-two polynomials (in total
$32$ predictors) to allow sophisticated propensity score models. In
the two RKHS regressions, we use the Gaussian kernel
\[
K(x, x') = \exp(-\gamma \|x - x' \|^2),~x,x' \in \mathbb{R}^4,
\]
with $\gamma$ equal to $0.2$ and $0.5$. After fitting a path of propensity score models (indexed
by step for forward stepwise and regularization parameter $\lambda$
for RKHS), for each strategy we choose the model that has the smallest
number of significant two-sample $t$-tests as described in
\Cref{sec:model-select-infer}. Finally, the standard errors and
confidence intervals by assuming homoscedasticity in \eqref{eq:tau-se}
and using a pilot outcome regression (predictors are the observed
$X$). Since a fairly sophisiticated propensity score model can be
fitted, we use $n = 1000$ samples and set $g(X,1) = g(X,0)$ to test all the methods.

\Cref{tab:ks-sim} shows the performance of the six different combinations of
loss function and adaptive strategy in the four simulation
settings. CBSR clearly outperforms Bernoulli likelihood. In almost all
scenarios and no matter what adaptive strategy is used, the root mean
squared error (RMSE) of CBSR is less than half of the RMSE of
Bernoulli likelihood. The confidence intervals obtained by using
Bernoulli likelihood also perform poorly. In many scenarios the actual
coverage is less than $50\%$, whereas the nominal coverage is
$95\%$. CBSR's confidence intervals have close to or over the nominal 95\%
coverage in almost all scenarios.

The two adaptive strategies (forward stepwise and RKHS) perform
similarly. When using CBSR as the loss function, forward stepwise
seems to have slightly smaller RMSE, but kernel methods can have the
better coverage in some scenarios. In practice, the user may want to choose an
adaptive strategy that is most convenient for the target
application. The strength and weakness of these methods are discussed
in \Cref{sec:extensions}.

\def\arraystretch{1}
\renewcommand{\tabcolsep}{5pt}
\begin{table}[tp]
\scriptsize
\begin{tabular}{|l|l|l|l|l|r|r|r|}
\hline
$f$ (true PS) & $g$ (true OR) & estimand & loss & strategy & bias & RMSE & coverage \\
\hline
linear & linear & ATE & Bernoulli & fstep  & $-1.27$ & $\phantom{0}2.43$ & $\phantom{0}50.5$ \\
 &  &  &  & kernel (0.2)  & $-2.77$ & $\phantom{0}3.18$ & $\phantom{0}22.5$ \\
 &  &  &  & kernel (0.5)  & $-3.05$ & $\phantom{0}3.45$ & $\phantom{0}17.5$ \\
 &  &  & CBSR & fstep  & $-0.24$ & $\phantom{0}0.98$ & $\phantom{0}90.0$ \\
 &  &  &  & kernel (0.2)  & $-0.50$ & $\phantom{0}1.16$ & $\phantom{0}90.5$ \\
 &  &  &  & kernel (0.5)  & $-1.41$ & $\phantom{0}1.77$ & $\phantom{0}63.0$ \\
 &  & ATT & Bernoulli & fstep  & $-2.92$ & $\phantom{0}6.28$ & $\phantom{0}55.5$ \\
 &  &  &  & kernel (0.2)  & $-7.30$ & $11.08$ & $\phantom{0}29.0$ \\
 &  &  &  & kernel (0.5)  & $-2.70$ & $\phantom{0}3.34$ & $\phantom{0}27.5$ \\
 &  &  & CBSR & fstep  & $-0.24$ & $\phantom{0}1.19$ & $\phantom{0}91.5$ \\
 &  &  &  & kernel (0.2)  & $-1.09$ & $\phantom{0}2.78$ & $\phantom{0}90.5$ \\
 &  &  &  & kernel (0.5)  & $-1.91$ & $\phantom{0}2.49$ &
 $\phantom{0}63.5$ \\
 & nonlinear & ATE & Bernoulli & fstep  & $-1.05$ & $\phantom{0}2.17$ & $\phantom{0}82.5$ \\
 &  &  &  & kernel (0.2)  & $-1.90$ & $\phantom{0}2.52$ & $\phantom{0}74.0$ \\
 &  &  &  & kernel (0.5)  & $-2.13$ & $\phantom{0}2.77$ & $\phantom{0}68.0$ \\
 &  &  & CBSR & fstep  & $-0.46$ & $\phantom{0}1.17$ & $\phantom{0}99.5$ \\
 &  &  &  & kernel (0.2)  & $-0.46$ & $\phantom{0}1.17$ & $100.0$ \\
 &  &  &  & kernel (0.5)  & $-1.10$ & $\phantom{0}1.62$ & $\phantom{0}96.0$ \\
 &  & ATT & Bernoulli & fstep  & $-0.93$ & $\phantom{0}3.87$ & $\phantom{0}87.5$ \\
 &  &  &  & kernel (0.2)  & $-3.16$ & $\phantom{0}6.64$ & $\phantom{0}65.5$ \\
 &  &  &  & kernel (0.5)  & $-0.05$ & $\phantom{0}1.82$ & $\phantom{0}94.0$ \\
 &  &  & CBSR & fstep  & $-0.49$ & $\phantom{0}1.37$ & $\phantom{0}99.0$ \\
 &  &  &  & kernel (0.2)  & $-0.27$ & $\phantom{0}2.05$ & $\phantom{0}99.0$ \\
 &  &  &  & kernel (0.5)  & $-0.59$ & $\phantom{0}1.83$ &
 $\phantom{0}99.5$ \\
\hline
nonlinear & linear & ATE & Bernoulli & fstep  & $-1.55$ & $\phantom{0}2.07$ & $\phantom{0}45.5$ \\
 &  &  &  & kernel (0.2)  & $-2.28$ & $\phantom{0}2.75$ & $\phantom{0}31.0$ \\
 &  &  &  & kernel (0.5)  & $-2.54$ & $\phantom{0}2.97$ & $\phantom{0}24.5$ \\
 &  &  & CBSR & fstep  & $-0.27$ & $\phantom{0}1.02$ & $\phantom{0}86.5$ \\
 &  &  &  & kernel (0.2)  & $-0.40$ & $\phantom{0}1.10$ & $\phantom{0}92.5$ \\
 &  &  &  & kernel (0.5)  & $-1.19$ & $\phantom{0}1.61$ & $\phantom{0}64.5$ \\
 &  & ATT & Bernoulli & fstep  & $-0.45$ & $\phantom{0}1.94$ & $\phantom{0}78.5$ \\
 &  &  &  & kernel (0.2)  & $-0.88$ & $\phantom{0}2.43$ & $\phantom{0}64.0$ \\
 &  &  &  & kernel (0.5)  & $-0.92$ & $\phantom{0}1.84$ & $\phantom{0}62.0$ \\
 &  &  & CBSR & fstep  & $-0.13$ & $\phantom{0}1.14$ & $\phantom{0}89.0$ \\
 &  &  &  & kernel (0.2)  & $-0.36$ & $\phantom{0}1.46$ & $\phantom{0}93.5$ \\
 &  &  &  & kernel (0.5)  & $-0.83$ & $\phantom{0}1.61$ &
 $\phantom{0}82.5$ \\
 & nonlinear & ATE & Bernoulli & fstep  & $-2.25$ & $\phantom{0}2.75$ & $\phantom{0}64.5$ \\
 &  &  &  & kernel (0.2)  & $-2.90$ & $\phantom{0}3.37$ & $\phantom{0}51.0$ \\
 &  &  &  & kernel (0.5)  & $-3.29$ & $\phantom{0}3.69$ & $\phantom{0}41.5$ \\
 &  &  & CBSR & fstep  & $-0.61$ & $\phantom{0}1.01$ & $100.0$ \\
 &  &  &  & kernel (0.2)  & $-0.73$ & $\phantom{0}1.26$ & $100.0$ \\
 &  &  &  & kernel (0.5)  & $-1.88$ & $\phantom{0}2.19$ & $\phantom{0}86.5$ \\
 &  & ATT & Bernoulli & fstep  & $-0.12$ & $\phantom{0}1.82$ & $\phantom{0}96.5$ \\
 &  &  &  & kernel (0.2)  & $-0.02$ & $\phantom{0}2.34$ & $\phantom{0}96.0$ \\
 &  &  &  & kernel (0.5)  & $-0.37$ & $\phantom{0}1.64$ & $\phantom{0}95.5$ \\
 &  &  & CBSR & fstep  & $-0.39$ & $\phantom{0}1.12$ & $100.0$ \\
 &  &  &  & kernel (0.2)  & $-0.35$ & $\phantom{0}1.46$ & $100.0$ \\
 &  &  &  & kernel (0.5)  & $-1.01$ & $\phantom{0}1.74$ & $\phantom{0}99.5$ \\
\hline
\end{tabular}
\caption{Performance of different loss functions combined with
  adaptive strategies---forward stepwise (fstep) and kernel method (Gaussian
  kernel with bandwidth parameter $0.2$ and $0.5$). In each case, the propensity
  score model is selected to minimize the number of significant
  covariate imbalance tests. Compared to the Bernoulli likelihood,
  maximizing the covariate balancing scoring rule (CBSR) reduces the root mean square error
  (RMSE) by more than a half for most settings. CBSR's confidence
  intervals also have the superior coverage (nominal level is $95\%$).}
\label{tab:ks-sim}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> tech-assump.tex <==
% \begin{assumption} (Unconfoundedness) \label{assump:unconfound}
%   $T \independent (Y(0),Y(1))|{X}$.
% \end{assumption}

% This assumption, which asserts that conditional on the observed
% covariates the treatment indicator is independent of the potential
% outcomes, is essential for identification of the average treatment
% effects \citep{Rosenbaum1983}.

\begin{assumption} (Distribution of ${X}$) \label{assump:X}
  The support of ${X}$ is a Cartesian product of compact
  intervals. The density of ${X}$ is bounded, and bounded away from
  $0$.
\end{assumption}

\begin{assumption} (Distribution of $Y(0),~Y(1)$) \label{assump:Y}
  The second moments of $Y(0)$ and $Y(1)$ exist and $g({X},0) =
  \mathrm{E}[Y(0)|{X}]$ and $g({X},1) = \mathrm{E}[Y(1)|{X}]$
  are continuously differentiable.
\end{assumption}

\begin{assumption} (Propensity score) \label{assump:ps}
  The propensity score $p({X}) = \mathrm{P}(T=1|{X})$ is
  continuously differentiable of order $s \ge 7d$ where $d$ is the
  dimension of ${X}$, and $p({x})$ is bounded away from $0$ and
  $1$.
\end{assumption}

\begin{assumption} (Sieve estimation) \label{assump:sieve}
  The nonparametric sieve logistic regression uses a power series with
  $m = n^{\nu}$ for some $1/(4(s/d-1)) < \nu < 1/9$.
\end{assumption}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

